Robust Vacuity for Branching Temporal Logic

There is a growing interest in techniques for detecting whether a logic specification is satisfied too easily, or vacuously. For example, the specification "every request is eventually followed by an acknowledgment" is satisfied vacuously by a system that never generates any requests. Vacuous satisfaction misleads users of model-checking into thinking that a system is correct. There are several existing definitions of vacuity. Originally, Beer et al. formalized vacuity as insensitivity to syntactic perturbation. However, this definition is only reasonable for vacuity in a single occurrence. Armoni et al. argued that vacuity must be robust -- not affected by semantically invariant changes, such as extending a model with additional atomic propositions. They show that syntactic vacuity is not robust for LTL, and propose an alternative definition -- trace vacuity. In this article, we continue this line of research. We show that trace vacuity is not robust for branching time logic. We refine it to apply uniformly to linear and branching time logic and to not suffer from the common pitfalls of prior definitions. Our new definition -- bisimulation vacuity -- is a proper non-trivial extension of both syntactic and trace vacuity. We discuss the complexity of detecting bisimulation vacuity, and give efficient algorithms to detect vacuity for several practically-relevant subsets of CTL*.

==> fig-model.tex <==
\begin{pspicture}(0,0)(3,1.2)\small
\cnodeput[framesep=0.28](1,0.5){a}{$p$}
\cnodeput[framesep=0.28](2.5,0.5){b}{$p$}

\psset{arrows=->}
\ncline{init}{a}
\ncline{a}{b}
\nccircle[angleA=0]{->}{b}{.3}
\nccircle[angleA=0]{->}{a}{.3}
\nput*{-45}{a}{$b_0$}
\nput*{-45}{b}{$b_1$}
\end{pspicture}  

%
%
%
%


==> mvvacuity.tex <==
\vspace{-0.1in}

\section{Vacuity Detection via 3-valued Model Checking}
\label{sec:vacu-detect-via}

In this section, we show that 3-valued model-checking provides a
uniform framework for studying vacuity detection. 

%
%
%
%


\vspace{-0.1in}

\subsection{3-Valued Model-Checking}
\label{sec:3-valued-model}

A 3-valued Kleene logic $\latstyle{3}$~\cite{kleene52}  is an extension
of a classical two-valued logic of \true and \false, with an
additional value \maybe, representing uncertainty. Propositional operators
in this logic, called Kleene operators, are defined via the \emph{truth} ordering $\below$, where
$\false \below \maybe \below \true$.  Intuitively, $a \below b$
indicates that $a$ is \emph{less true} than $b$. Conjunction and
disjunction are given by meet (minimum) and join (maximum) operators
of the truth ordering, respectively. Negation is defined as: $\neg
\true = \false$, $\neg \false = \true$, and $\neg \maybe = \maybe$.
Kleene logic preserves most of the laws of classical logic, such as De
Morgan laws ($\neg (a \land b) = \neg a \lor \neg b$), and an
involution of negation ($\neg \neg a = a$), but not the laws of
excluded middle ($a \lor \neg a = \true$) and non-contradiction ($\neg
a \land a = \false$).  The values of Kleene logic can also be ordered
according to the \emph{information} ordering $\infoleq$, where
\maybe $\infoleq$ \true and \maybe $\infoleq$ \false.  That is,
\maybe contains the least amount of information, whereas \true and \false
are incomparable.

Model-checking is extended to the 3-valued logic by allowing models
with uncertain information, represented by atomic propositions with
value $\maybe$. Formally, a model is a 3-valued \kripke structure $K =
(AP, S, S_0, R, I)$, where $AP$, $S$, $S_0$, and $R$ are classical,
and $I$ is a function $S \times A \rightarrow \latstyle{3}$. 
Any classical \kripke structure is simply a 3-valued \kripke structure
that does not make use of \maybe values.  Adding 3-valued transitions
to 3-valued Kripke structures does not increase their expressive power~\cite{godefroid03}.

%
%
%
%
%
%

The semantics of \ctlast is extended to 3-valued models by reinterpreting
propositional operators.
For example, 
$||EX p||(s) = \Lor_{t \in S} R(s, t) \land ||p||(t)$, where
$\Lor$ and $\land$ are Kleene.  In classical
models, the 3-valued and two-valued semantics of \ctlast coincide.
In what follows, we refer to this semantics as \emph{compositional}.

The information ordering $\infoleq$ is extended to 3-valued \kripke
structures providing a completeness preorder that connects classical and
3-valued \kripke structures. Intuitively, a 3-valued \kripke structure
$K$ is more complete than $K'$, written $K' \infoleq K$, if the information
contained in $K'$ is less certain than that in $K$.  In this case,
$K$ is a \emph{refinement} of $K'$. 
%

\vspace{-0.1in}

\begin{definition}\cite{bruns99}
  \label{def:refinement}
  A relation $\rho \subseteq S \times S'$ is a refinement between
  3-valued \kripke structures $K$ and $K'$ iff $\rho(s,s')$ implies

\vspace{-0.05in}

  \begin{enumerate}
   \item $\A{p \in AP} I(s, p) \infoleq I'(s', p)$
   \item $\A{t \in S} R(s, t) \limp \E{t' \in S'} R'(s', t') \land \rho(t,t')$
   \item $\A{t' \in S'} R'(s', t') \limp \E{t \in S} R(s,t) \land \rho(t,t')$
  \end{enumerate}
\end{definition}

\vspace{-0.1in}

\noindent
A state $s$ is refined by a state $s'$ ($s \infoleq s'$) if there
exists a refinement $\rho$ containing $(s, s')$. A \kripke structures
$K$ is refined by $K'$ ($K \infoleq K'$) if there exists a refinement
$\rho$ relating their initial states: $\A{s \in S_0}\E{s' \in S'_0}
\rho(s,s')$ and $\A{s' \in S'_0}\E{s \in S_0} \rho(s,s')$.
Intuitively, $K$ refines $K'$ if $K$ is bisimilar to $K'$, provided we ignore
the uncertain (\maybe) atomic propositions of $K'$. In
particular, bisimulation and refinement coincide on classical
structures. 

\vspace{-0.05in}

\begin{theorem}\cite{bruns99}
  \label{thm:refinement-characterization}
  For 3-valued \kripke structures $K$ and $K'$ and a \ctlast formula
  $\varphi$, $K \infoleq K'$ implies $||\varphi||^K \infoleq
  ||\varphi||^{K'}$, i.e., refinement preserves 3-valued \ctlast.
\end{theorem}

\vspace{-0.05in}

\noindent
The refinement relation relates 3-valued and classical models. For a
3-valued \kripke structure $K$, let $\C(K)$ denote the set of
\emph{completions} of $K$ -- the set of all classical \kripke
structures that refine $K$. For any completion $K' \in \C(K)$, the
structure $K$ can be seen as less precise than $K'$ in the sense that
any \ctlast formula that evaluates to a definite value (either \true
or \false) in $K$, evaluates to the same value in $K'$.  That is, for
any $K' \in \C(K)$ and any \ctlast formula $\varphi$,
$  (||\varphi||^K = \true)  \limp (||\varphi||^{K'} = \true)$ and
$  (||\varphi||^K = \false) \limp (||\varphi||^{K'} = \false)$.
The converse, however, does not hold is in general. For example, the
formula $p \lor \neg p$ is \true in any classical model, yet its value
is $\maybe$ in any state of a 3-valued model that assigns $\maybe$ to
$p$ (i.e., $p \lor \neg p = \maybe \lor \neg \maybe = \maybe \lor
\maybe = \maybe)$.

To address this imprecision of compositional semantics, Bruns and
Godefroid~\cite{bruns00} have introduced an alternative semantics,
calling it \emph{thorough}.

\vspace{-0.1in}

\begin{definition}~\cite{bruns00}
  \label{def:thorough-semantics}
  Let $K$ be a 3-valued \kripke structure, and $\varphi$ a \ctlast
  formula. The value of $\varphi$ in $K$ under thorough semantics
  $||\varphi||_t^K$ is: \true iff $\varphi$ holds in every completion
  of $K$, \false if it is \false in every completion, and \maybe
  otherwise.
%
%
%
%
%
%
%
%
\end{definition}

\vspace{-0.1in}

Thorough semantics always produces more exact answers than
compositional, i.e., for any 3-valued \kripke structure $K$ and a
\ctlast formula $\varphi$, $||\varphi||^K \infoleq
||\varphi||_t^K$. This additional precision comes at a price of
complexity: model-checking a given branching temporal logic formula
under compositional semantics is in the same complexity class as
classical model-checking; however, its model-checking complexity under
thorough semantics is as hard as satisfiability~\cite{bruns00}.

\vspace{-0.1in}

\subsection{Vacuity Detection via 3-valued Model-Checking}
\label{sec:vacu-detect-via-1}
In this section, we show that vacuity detection is closely related
to 3-valued model-checking under thorough semantics.

Let $K$ be a \kripke structure, and let $K_x$ be a 3-valued \kripke
structure obtained from $K$ by: (a) adding to $K$ a new atomic
proposition $x$, and (b) setting the value of $x$ to \maybe in every
state. The set $\C(K_x)$ of completions of $K_x$ is equivalent to the
set of \kripke structures which are $\{x\}$-bisimilar to $K$.

\vspace{-0.1in}

\begin{theorem}
  \label{thm:completion-xbisimilarity}
  Let $K$ be a \kripke structure, and $K_x$ be as described above. Then,
  $K' \in \C(K_x)$ iff $K'$ is $\{x\}$-bisimilar to $K$.
\end{theorem}

\vspace{-0.1in}

\noindent This theorem
suggests the following
reduction from vacuity detection to 3-valued model-checking:

\vspace{-0.1in}

\begin{tabbing}
blah \= if I have \= if\=\kill
\>  To check
whether a formula $\varphi$ is $\psi$-vacuous in $K$: \\
\> \> Construct a 3-valued \kripke structure $K_x$.\\
\> \> Model-check $\varphi[\psi \subst x]$ in $K_x$ under thorough semantics.\\
\>  \> {\bf if}  $||\varphi[\psi \subst x]||_t^{K_x} \in \{\true, \false\}$\\
\> \> \> {\bf then} {\bf return} ``$\varphi$ is $\psi$-vacuous''\\
\> \> {\bf else} {\bf return} ``$\varphi$ is not $\psi$-vacuous''.
\end{tabbing}

\vspace{-0.1in}

\noindent
The reduction in
the other direction, i.e., from 3-valued model-checking to vacuity
detection, is also possible, but is outside the scope of this
paper.

As the result of this reduction, any advance in
3-valued model-checking is also applicable to vacuity detection. For
example, the complexity of thorough semantics model-checking for \ctl
and \ctlast is known to be EXPTIME- and
2EXPTIME-comp-\\lete~\cite{bruns00}, respectively, which provides an
alternative proof of the first part of
Theorem~\ref{thm:vacuity-complexity}. 
For another notable example, consider \actlast persistence properties~\cite{manna92}, i.e.,
properties of the form $AFG p$.  These correspond to co-\buchi automata,
and the complexity of model-checking these properties under
thorough semantics is linear in the
size of the model~\cite{godefroid02}. Thus, for such properties, the
complexity of vacuity detection is the same as that of  model-checking.

Note that since thorough semantics is more precise than compositional, 
model-checking $\varphi[\psi \subst x]$ in $K_x$ under
compositional semantics yields a sound approximation to vacuity
detection. If $||\varphi[\psi \subst x]||^{K_x}$ is either \true or
\false, then $\varphi$ is $\psi$-vacuous; otherwise, the result of the
model-checking is \maybe, which gives no information about vacuity.
Moreover, our previous work~\cite{gurfinkel03b} showed that if $\psi$
occurs in $\varphi$ with pure polarity, then compositional semantics
reduces to checking whether $||\varphi[\psi \subst \true]||^K =
||\varphi[\psi \subst \false]||^K$. Thus, by
Theorems~\ref{thm:monotone-vacuity}
and~\ref{thm:syntactic-monotonicity}, compositional semantics provides
a sound and complete algorithm for vacuity detection in subformulas of pure polarity.

An additional benefit of the reduction enables the use of 3-valued model-checkers,
which are arguably necessary for combining model-checking and abstraction~\cite{godefroid02,shoham03}, to
solve the vacuity detection problem.
Moreover, witnesses and counterexamples, produced by such
model-checkers, can be used to explain why a given formula is deemed
to be (non-)vacuous.  To our knowledge, a 3-valued
model-checker with thorough semantics has not been implemented.  Further,
we are not aware of an algorithm for generating witnesses and counterexamples
in this case, but it appears to be  equivalent to logic synthesis
and  thus very expensive.  However, compositional 3-valued model-checkers,
such as $\Chi$Chek~\cite{chechik02b}, have been implemented, and their
witnesses and counterexamples
have a natural correspondence to witnesses for
non-vacuity~\cite{beer01}.  This connection  has been explored in our previous
work~\cite{gurfinkel04a}.
%
%
%
%
%
%

Finally, reducing vacuity detection to 3-valued model-checking makes
it easier to explore the combination of vacuity detection with various
abstraction techniques, as we explore in the next section.

%
%
%
%

